Detecting Label Errors by using Pre-Trained Language Models

We show that large pre-trained language models are inherently highly capable of identifying label errors in natural language datasets: simply examining out-of-sample data points in descending order of fine-tuned task loss significantly outperforms more complex error-detection mechanisms proposed in previous work. To this end, we contribute a novel method for introducing realistic, human-originated label noise into existing crowdsourced datasets such as SNLI and TweetNLP. We show that this noise has similar properties to real, hand-verified label errors, and is harder to detect than existing synthetic noise, creating challenges for model robustness. We argue that human-originated noise is a better standard for evaluation than synthetic noise. Finally, we use crowdsourced verification to evaluate the detection of real errors on IMDB, Amazon Reviews, and Recon, and confirm that pre-trained models perform at a 9-36% higher absolute Area Under the Precision-Recall Curve than existing models.

==> tables/error_examples_long.tex <==
\begin{table*}[Ht!]
\centering
\small
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{llp{8.5cm}p{3.5cm}}
\toprule
\textbf{\specialcell{Dataset\\Label}} & \textbf{Error?} & \textbf{Text} & \textbf{Explanation} \\
\midrule
% Negative & Non-Err. & Masterpiece. Carrot Top blows the screen away. Never has one movie captured the essence of the human spirit quite like ``Chairman of the Board.'' 10/10... don't miss this instant classic. & The review is sarcastic. \\ 
% Neutral & Error & This app was great for someone who has stylus but really pointless when you're using your finger. I recommend it for people who own a stylus and write small and neat. & The review may be neutral overall, but the experts and the New MTurk protocol \\ 
Neutral & Non-Err. & I've had this case for about 4-5 months now and it has already broken from light use. It also had trouble holding my ipad up unless I really worked to make sure it didn't fall over. However, before it broke I really loved it. Great alternative to a Smart Cover. &  The description is balanced between positive and negative. \\
% Neutral & Error & It's like blowing up a balloon, only there's no way to pinch off the flow, so it just blows right out.  Too bad, because the removable cover is neat!  Oh, and the description says its weight is 2 pounds.  Uhn uhn, try 3.5 ounces. \\
Neutral & Error & The new design only has a thin layer of cellulose sponge material.  It will not last as long.  Already showing signs of wearing out.  The picture does not represent the item received. & The description is overwhelmingly negative. \\
Positive & Non-Err. & This is a great film for pure entertainment, nothing more and nothing less. It's enjoyable, and a vaguely feel-good movie. A minor, but nonetheless irritating thing about the movie is that we don't know why Justine and Chas broke up. Okay, most first relationships don't work for one reason or another, but they more or less seemed like a nice couple. In a nutshell, it's worth a watch to escape reality. & The review ultimately recommends the film as ``worth a watch.'' \\
Positive & Error & It is really unfortunate that a movie so well produced turns out to be such a disappointment. I thought this was full of (silly) cliches that it basically tried to hard. It had all sorts of differences that it tried to tie together (not a bad thing in itself) but the result is at best awkward, but in fact ridiculous--too many clashes that wouldn't really happen. Then the end of the movie--the last 10 minutes--ruined all the rest. At first I thought Xavier was OK but with retrospect I think he was pretty bad. And that's all really too bad, because technically it was really good, and the soundtrack was great too. So the form was good, but the content pretty horrible. & The review makes positive comments but only to contrast them with the conclusion, which is ultimately negative. \\
Negative & Error & The ending made my heart jump up into my throat. I proceeded to leave the movie theater a little jittery. After all, it was nearly midnight. The movie was better than I expected. I don't know why it didn't last very long in the theaters or make as much money as anticipated. Definitely would recommend. & The review ultimately recommends the film, with a score of 4/10, which is on the borderline of the negative range. \\ 
Negative & Non-Err. & Somehow, this documentary about Miles manages to include very little music and no complete tunes. Though Miles appears in the film, 95\% of the interviews are other folks, not Miles. There are huge chronological gaps, many aspects of his life (his childhood prodigy, his drug addiction) are skipped or glossed over, and you'll learn little about what made the man and his contribution to music so groundbreaking. Skip it. & The review is entirely critical \\ 
\bottomrule
\end{tabular}
\caption{(Placeholder) Some examples of typical label noise.}
\label{detailed-ea-edu}
\end{table*}

==> unused/aupr_long_table_transpose.tex <==
\begin{table*}
\small
\centering
\begin{tabular}{l|ccccc|ccccc|ccccc}
& \multicolumn{5}{|c|}{Area Under Precision-Recall Curve} & \multicolumn{5}{|c|}{Precision at Err\%} & \multicolumn{5}{|c}{Recall at 2 $\cdot$ Err\%} \\ \hline
& H & CL & FML & FME & \specialcell{FME\\+CL} & H & CL & FML & FME & \specialcell{FME\\+CL} & H & CL & FML & FME & \specialcell{FME\\+CL} \\ \hline
IMDB & - & 0.24 & 0.57 & \textbf{0.60} & 0.20 & - & 0.42 & 0.69 & \textbf{0.70} & - & - & - & - & - & - \\ 
Amazon & - & xxx & 0.39 & 0.40 & 0.40 & - & xxx & 0.64 & 0.66 & 0.66 & - & - & - & - & - \\ 
TweetNLP-5 & 0.30 & 0.30 & 0.66 & 0.68 & 0.68 & 0.30 & 0.30 & 0.67 & 0.65 & 0.65 & 0.58 & 0.58 & 0.88 & 0.88 & 0.88 \\ 
TweetNLP-M & 0.40 & 0.41 & \textit{0.48} & \textit{0.48} & \textit{0.48} & 0.33 & 0.38 & 0.44 & 0.44 & 0.44  & 0.75 & 0.75 & 0.70 & 0.69 & 0.69 \\ 
SNLI-5 & 0.20 & 0.17 & 0.54 & 0.61 & 0.62 & 0.25 & 0.22 & 0.54 & 0.60 & 0.60 & 0.37 & 0.36 & 0.78 & 0.80 & 0.80 \\ 
% Recon & 12 & 14 & \textbf{16} & 35  \\ 
\end{tabular}
\caption{Truncated Area under the Precision-Recall Curve (AUPR) for each method on real data using direct verification of label errors.}
\label{tab:aupr_precision_recall_all_transpose}
\end{table*}

==> unused/cleanval_gain.tex <==
\begin{table}
    \small
    \centering
    \begin{tabular}{l|l|ccc|c|c}
        \multirow{2}{*}{Dataset} & \multirow{2}{*}{Noise} & \multicolumn{3}{|c|}{Noisy Train} & \multirow{2}{*}{Oracle} & \multirow{2}{*}{Gain} \\ \cline{3-5}
        & & NV & CV & OR & & \\ \hline
        IMDB & CL 5\% & 90.08 & 95.12 & 95.12 & 95.60 & 5.04 \\ \hline
        Amazon & CL 5\% & 88.32 & 90.72 & 90.80 & 91.04 & 2.40 \\ \hline
        \multicolumn{2}{l|}{TweetNLP-5 (5\%)} & 89.78 & 93.30 & 93.53 & 94.43 & 3.52 \\ \hline 
        \multicolumn{2}{l|}{TweetNLP-M (20\%)} & 89.33 & 88.47 & 82.03 & 93.47 & 0.86 % \\ \hline 
        % RECON CUTOUT
        % Recon & Real 20\% & XXX & XXX & XXX & XXX
    \end{tabular}
    \caption{We report the accuracy of each model on the respective task for each dataset. The Noise column describes the mechanism that generates the label errors and the approximate proportion of label errors, across training, validation, and test. The columns refer to using noisy training data with noisy validation and noisy training data with a validation dataset that has been cleaned using our methods. The Oracle column refers to using training, validation, and test sets that are clean. The Gain column compares the difference between the NV and CV columns under Noisy Train.}
    % \caption{XXX}
    \label{tab:t5-cleanval-gain}
\end{table}


==> unused/loss-allruns.tex <==
\begin{figure}
\begin{tikzpicture}
\begin{axis}[%
scatter/classes={%
    a={mark=o,draw=black}}]
\addplot[scatter,only marks,%
    scatter src=explicit symbolic]%
table[meta=label] {
x y label
1 4.3 a
2 5.1 a
3 5.7 a
4 6.3 a
5 6.8 a
6 7.1 a
7 7.2 a
8 7.2 a
9 7.2 a
10 7.2 a
11 7.5 a
12 7.8 a
    };
\end{axis}
\end{tikzpicture}
\caption{test fig please ignore}
\label{arch}
\end{figure}


==> unused/tmp.tex <==

\section{Introduction}
Approaches to learning with mislabelings generally fall into two categories: model-centric methods and data-centric methods. Model-centric methods aim to improve the model and training techniques without modifying the underlying data, such as through robust learning. However, much less work has been invested in data-centric approaches, which addresses important complementary issues that model-centric approaches are not designed to handle. 
Data-centric methods to improve the underlying data can be especially valuable for smaller datasets \citep{ng2021data}. Second, data-centric methods can assist not only with training models, but also with evaluating models. In many commonly used NLP benchmarks, such as IMDB and Amazon Reviews, the presence of mislabelings has been shown to destabilize model performance \citep{northcutt2021pervasive}. In other words, mislabelings in the test set can be misleading as to which methods actually improve performance.

However, existing methods for identifying mislabelings in natural language datasets generally have not taken advantage of recent advances in pre-trained large language models. We hypothesize that pre-training on other large datasets can improve detection of mislabelings on a particular task. In order to evaluate our method, we replicate crowdsourcing methods for validating hypothesized mislabelings. We also contribute a novel method for constructing realistic synthetic mislabelings from existing crowdsource data. We show that a straightforward application of large language models outperforms existing methods for identifying mislabelings on natural language datasets.

\section{Related Work}
Efforts to identify and correct incorrect labels have focused on studying noise in which the reported label originates from an artificial type of corruption applied to a true label. For example, \citet{hendrycks2018using} applies artificial corruption to underlying datasets (such as IMDB and Gimpel), in the context of training data. The experiments use artificial corruption, such as flipping to a random class. \citet{xia2020extended} uses a fixed error rate for each class and also focuses on training. 

Correcting underlying labels is a more data-centric approach and has an additional benefit that model-centric methods fail to address. Label errors in validation and testing, which have been shown to destabilize model performance \cite{northcutt2021pervasive}, and a method that corrects labels can correct them across training and held-out data.

A data-centric should also focus on the particular mechanisms that introduce errors to labels. Such mislabelings are distributed differently from artificially corrupted labels. Confident learning, CoNLL

% \begin{table}
% \small
% \centering
% \begin{tabular}{l|l|ccc|c}
% \hline
% \multicolumn{2}{c}{\multirow{2}{*}{\specialcell{Orig. MTurk Labels}}} & \multicolumn{3}{|c|}{New MTurk Labels} & \multirow{2}{*}{\specialcell{Orig.\\Total}} \\ \cline{3-5}
% \multicolumn{2}{c|}{} & C & NA & NE & \\ \hline
% \multirow{4}{*}{IMDB} & Corr. & 105 & 44 & 24 & 173\\ \cline{2-6}
% & Non-Agr. & 75 & 252 & 225 & \textbf{552} \\ \cline{2-6}
% & Non-Err. & 3 & 62 & 520 & 585 \\ \hline 
% & {New Total} & 183 & \textbf{358} & 769 & 1310 \\ \hline

% \multicolumn{2}{c}{\multirow{2}{*}{\specialcell{Orig. MTurk Labels}}} & \multicolumn{3}{|c|}{New MTurk Labels} & \multirow{2}{*}{\specialcell{Orig.\\Total}} \\ \cline{3-5}
% \multicolumn{2}{c|}{} & C & NA & NE & \\ \hline
% \multirow{4}{*}{Amazon} & Corr.  & 142 & 43 & 117 & 302 \\ \cline{2-6}
% & Non-Agr. & 140 & 79 & 211 & \textbf{430} \\ \cline{2-6}
% & Non-Err. & 75 & 31 & 162 & 268 \\ \hline
% & New Total & 357 & \textbf{153} & 490 & 1000 \\ 
% \end{tabular}
% \caption{For the mislabelings hypothesized by Confident Learning, the number of correctable, non-agreement, and non-errors identified by the original \citet{northcutt2021confident} MTurk protocol and by the new protocol, respectively.}
% \label{tab:turk-eval-long}
% \end{table}

% \begin{table}
% \small
% \centering
% \begin{tabular}{l|l|ccc||c}
% \hline
% \multicolumn{2}{c}{} & \multicolumn{3}{|c||}{New MTurk Labels}  \\ \hline
% \multicolumn{2}{c|}{Orig. MTurk Labels} & C & NA & NE & Orig. Total \\ \hline
% \multirow{4}{*}{IMDB} & Corr. & 105 & 44 & 24 & 173\\ \cline{2-6}
% & Non-Agr. & 75 & 252 & 225 & \textbf{552} \\ \cline{2-6}
% & Non-Err. & 3 & 62 & 520 & 585 \\ \hline \hline
% & {New Total} & 183 & \textbf{358} & 769 & 1310 \\ \hline \hline

% \multicolumn{2}{c}{} & \multicolumn{3}{|c||}{New MTurk Labels} \\ \hline
% \multicolumn{2}{c|}{Orig. MTurk Labels}  & C & NA & NE & Orig. Total \\ \hline
% \multirow{4}{*}{Amazon} & Corr.  & 142 & 43 & 117 & 302 \\ \cline{2-6}
% & Non-Agr. & 140 & 79 & 211 & \textbf{430} \\ \cline{2-6}
% & Non-Err. & 75 & 31 & 162 & 268 \\ \hline \hline
% & New Total & 357 & \textbf{153} & 490 & 1000 \\ 
% \end{tabular}
% \caption{For the mislabelings hypothesized by Confident Learning, the number of correctable, non-agreement, and non-errors identified by the original \citet{northcutt2021confident} MTurk protocol and by the new protocol, respectively.}
% \label{tab:turk-eval-long}
% \end{table}

